Evaluating the Impact of Social Determinants on Health Prediction in the Intensive Care Unit

Social determinants of health (SDOH) -- the conditions in which people live, grow, and age -- play a crucial role in a person's health and well-being. There is a large, compelling body of evidence in population health studies showing that a wide range of SDOH is strongly correlated with health outcomes. Yet, a majority of the risk prediction models based on electronic health records (EHR) do not incorporate a comprehensive set of SDOH features as they are often noisy or simply unavailable. Our work links a publicly available EHR database, MIMIC-IV, to well-documented SDOH features. We investigate the impact of such features on common EHR prediction tasks across different patient populations. We find that community-level SDOH features do not improve model performance for a general patient population, but can improve data-limited model fairness for specific subpopulations. We also demonstrate that SDOH features are vital for conducting thorough audits of algorithmic biases beyond protective attributes. We hope the new integrated EHR-SDOH database will enable studies on the relationship between community health and individual outcomes and provide new benchmarks to study algorithmic biases beyond race, gender, and age.

==> tables/ex_sdoh.tex <==
\begin{table*}[!b]
\centering
\caption{Five Key SDOH Domains and Example Features}
\label{ex_sdoh}
\resizebox{0.75\textwidth}{!}{%
\begin{tabular}{@{}ll@{}}
\toprule
\multicolumn{1}{c}{SDOH Domain}    & \multicolumn{1}{c}{Features}                                                                                                                                                                                        \\ \midrule
Economic Stability                 & \begin{tabular}[c]{@{}l@{}}Median household income\\ Percentage of households receiving food stamps\end{tabular}                                                              \\ \midrule
Education Access and Quality       & \begin{tabular}[c]{@{}l@{}}Percentage of teens and adults who are unemployed and not in school\\ Percentage of population with an advanced degree\end{tabular} \\ \midrule
Healthcare Access and Quality      & \begin{tabular}[c]{@{}l@{}}Percentage of population with direct-purchase health insurance only\\ Distance to the nearest health clinic\end{tabular}                  \\ \midrule
Neighborhood and Built Environment & \begin{tabular}[c]{@{}l@{}}Percentage of household built before 1979\\ Total number of convenience stores\end{tabular}                                                  \\ \midrule
Social and Community Context       & \begin{tabular}[c]{@{}l@{}}Total civilian noninstitutionalized population\\ Percentage of population who are not U.S. citizens\end{tabular}                                                    \\ \bottomrule
\end{tabular}%
}
\end{table*}

==> tables/tasks.tex <==
\begin{table}[htp]
\caption{Proportion of positive and negative labels across the three prediction tasks.}
\resizebox{0.95\columnwidth}{!}{%
\begin{tabular}{@{}ccc@{}}
\toprule
\multicolumn{1}{c}{Prediction Task} & \begin{tabular}[c]{@{}c@{}}Number of\\ Admissions \end{tabular} & \begin{tabular}[c]{@{}c@{}}Label Distribution\\ (Positive / Negative)\end{tabular} \\ \midrule
In-hospital Mortality               & 54,380             & 0.91 / 0.09                                                                        \\
30-Day Readmission                  & 49,646             & 0.94 / 0.06                                                                        \\
One-Year Mortality                  & 49,646             & 0.80 / 0.20                                                                        \\ \bottomrule
\end{tabular}%
}
\end{table}


==> tables/vulnearble_pop_one_year_mort.tex <==
\begin{longtable}{l|llrrrrrrr}
\caption{Comparison of model performance for classifiers trained on different data modalities to predict \textit{one-year mortality} for different patient populations. See \autoref{cohort_stats} for characteristics of the different patient populations.}
\label{apd:one_year_mort}\\
\toprule
Model        &       Patient                        & Feature Set &  AUROC &  AUPRC &   ECE &   FPR &  Recall &  Precision &  Specificity \\
\midrule
\endfirsthead
\toprule
Model        &       Patient                        & Feature Set &  AUROC &  AUPRC &   ECE &   FPR &  Recall &  Precision &  Specificity \\
\midrule
\endhead
\midrule
\multicolumn{10}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\endlastfoot
\multirow{42}{*}{Logistic Regression} & \multirow{7}{*}{All ICU} & SDOH &   0.55 &   0.22 &  0.30 &  0.45 &    0.53 &       0.23 &         0.55 \\
        &                               & Tabular &   0.82 &   0.52 &  0.22 &  0.26 &    0.75 &       0.42 &         0.74 \\
        &                               & Tabular+SDOH &   0.82 &   0.53 &  0.21 &  0.26 &    0.75 &       0.42 &         0.74 \\
        &                               & Notes &   0.83 &   0.55 &  0.18 &  0.23 &    0.72 &       0.44 &         0.77 \\
        &                               & Notes+SDOH &   0.83 &   0.55 &  0.19 &  0.24 &    0.74 &       0.44 &         0.76 \\
        &                               & All &   0.85 &   0.59 &  0.18 &  0.23 &    0.77 &       0.46 &         0.77 \\
        &                               & All+SDOH &   0.85 &   0.59 &  0.18 &  0.23 &    0.77 &       0.46 &         0.77 \\
\cline{2-10}
        & \multirow{7}{*}{All Diabetic} & SDOH &   0.53 &   0.25 &  0.26 &  0.46 &    0.49 &       0.25 &         0.54 \\
        &                               & Tabular &   0.77 &   0.49 &  0.19 &  0.28 &    0.67 &       0.43 &         0.72 \\
        &                               & Tabular+SDOH &   0.76 &   0.49 &  0.19 &  0.28 &    0.68 &       0.43 &         0.72 \\
        &                               & Notes &   0.80 &   0.55 &  0.16 &  0.23 &    0.67 &       0.48 &         0.77 \\
        &                               & Notes+SDOH &   0.79 &   0.54 &  0.16 &  0.24 &    0.65 &       0.47 &         0.76 \\
        &                               & All &   0.81 &   0.57 &  0.15 &  0.23 &    0.69 &       0.48 &         0.77 \\
        &                               & All+SDOH &   0.80 &   0.56 &  0.14 &  0.23 &    0.67 &       0.48 &         0.77 \\
\cline{2-10}
        & \multirow{7}{*}{Black Diabetic} & SDOH &   0.51 &   0.27 &  0.23 &  0.42 &    0.43 &       0.27 &         0.58 \\
        &                               & Tabular &   0.72 &   0.49 &  0.16 &  0.26 &    0.59 &       0.45 &         0.74 \\
        &                               & Tabular+SDOH &   0.76 &   0.53 &  0.16 &  0.24 &    0.63 &       0.49 &         0.76 \\
        &                               & Notes &   0.72 &   0.51 &  0.16 &  0.24 &    0.55 &       0.45 &         0.76 \\
        &                               & Notes+SDOH &   0.67 &   0.43 &  0.12 &  0.20 &    0.43 &       0.44 &         0.80 \\
        &                               & All &   0.77 &   0.54 &  0.12 &  0.21 &    0.56 &       0.49 &         0.79 \\
        &                               & All+SDOH &   0.72 &   0.47 &  0.12 &  0.22 &    0.53 &       0.46 &         0.78 \\
\cline{2-10}
        & \multirow{7}{*}{Elderly Diabetic} & SDOH &   0.49 &   0.34 &  0.16 &  0.53 &    0.50 &       0.33 &         0.47 \\
        &                               & Tabular &   0.70 &   0.54 &  0.14 &  0.34 &    0.62 &       0.49 &         0.66 \\
        &                               & Tabular+SDOH &   0.70 &   0.54 &  0.14 &  0.34 &    0.65 &       0.50 &         0.66 \\
        &                               & Notes &   0.74 &   0.60 &  0.12 &  0.31 &    0.64 &       0.52 &         0.69 \\
        &                               & Notes+SDOH &   0.72 &   0.57 &  0.09 &  0.27 &    0.56 &       0.52 &         0.73 \\
        &                               & All &   0.74 &   0.59 &  0.11 &  0.30 &    0.64 &       0.53 &         0.70 \\
        &                               & All+SDOH &   0.73 &   0.58 &  0.11 &  0.30 &    0.61 &       0.51 &         0.70 \\
\cline{2-10}
        & \multirow{7}{*}{Female Diabetic} & SDOH &   0.51 &   0.26 &  0.25 &  0.42 &    0.46 &       0.26 &         0.58 \\
        &                               & Tabular &   0.75 &   0.47 &  0.19 &  0.30 &    0.65 &       0.41 &         0.70 \\
        &                               & Tabular+SDOH &   0.74 &   0.46 &  0.19 &  0.31 &    0.67 &       0.41 &         0.69 \\
        &                               & Notes &   0.78 &   0.52 &  0.17 &  0.22 &    0.62 &       0.48 &         0.78 \\
        &                               & Notes+SDOH &   0.75 &   0.49 &  0.10 &  0.19 &    0.53 &       0.48 &         0.81 \\
        &                               & All &   0.78 &   0.53 &  0.14 &  0.23 &    0.61 &       0.46 &         0.77 \\
        &                               & All+SDOH &   0.77 &   0.52 &  0.14 &  0.24 &    0.61 &       0.45 &         0.76 \\
\cline{2-10}
        & \multirow{7}{*}{Non-English Speaking Diabetic} & SDOH &   0.54 &   0.27 &  0.24 &  0.36 &    0.40 &       0.28 &         0.64 \\
        &                               & Tabular &   0.72 &   0.46 &  0.19 &  0.32 &    0.63 &       0.40 &         0.68 \\
        &                               & Tabular+SDOH &   0.73 &   0.49 &  0.20 &  0.34 &    0.64 &       0.39 &         0.66 \\
        &                               & Notes &   0.75 &   0.47 &  0.10 &  0.19 &    0.45 &       0.45 &         0.81 \\
        &                               & Notes+SDOH &   0.72 &   0.41 &  0.10 &  0.19 &    0.45 &       0.44 &         0.81 \\
        &                               & All &   0.74 &   0.49 &  0.15 &  0.25 &    0.54 &       0.42 &         0.75 \\
        &                               & All+SDOH &   0.73 &   0.49 &  0.20 &  0.34 &    0.64 &       0.39 &         0.66 \\
\cline{1-10}
\cline{2-10}
\multirow{42}{*}{Random Forest} & \multirow{7}{*}{All ICU} & SDOH &   0.55 &   0.23 &  0.29 &  0.43 &    0.50 &       0.23 &         0.57 \\
        &                               & Tabular &   0.82 &   0.53 &  0.20 &  0.26 &    0.74 &       0.42 &         0.74 \\
        &                               & Tabular+SDOH &   0.82 &   0.52 &  0.21 &  0.26 &    0.74 &       0.42 &         0.74 \\
        &                               & Notes &   0.77 &   0.46 &  0.25 &  0.32 &    0.72 &       0.36 &         0.68 \\
        &                               & Notes+SDOH &   0.77 &   0.47 &  0.25 &  0.32 &    0.71 &       0.36 &         0.68 \\
        &                               & All &   0.82 &   0.53 &  0.24 &  0.29 &    0.78 &       0.40 &         0.71 \\
        &                               & All+SDOH &   0.82 &   0.53 &  0.24 &  0.29 &    0.78 &       0.41 &         0.71 \\
\cline{2-10}
        & \multirow{7}{*}{All Diabetic} & SDOH &   0.53 &   0.26 &  0.26 &  0.45 &    0.49 &       0.26 &         0.55 \\
        &                               & Tabular &   0.78 &   0.50 &  0.16 &  0.24 &    0.64 &       0.46 &         0.76 \\
        &                               & Tabular+SDOH &   0.78 &   0.51 &  0.16 &  0.24 &    0.63 &       0.46 &         0.76 \\
Random Forest        &                               & Notes &   0.75 &   0.49 &  0.21 &  0.31 &    0.67 &       0.41 &         0.69 \\
        &                               & Notes+SDOH &   0.75 &   0.50 &  0.21 &  0.30 &    0.66 &       0.41 &         0.70 \\
        &                               & All &   0.80 &   0.54 &  0.20 &  0.27 &    0.70 &       0.45 &         0.73 \\
        &                               & All+SDOH &   0.79 &   0.53 &  0.20 &  0.27 &    0.72 &       0.46 &         0.73 \\
\cline{2-10}
        & \multirow{7}{*}{Black Diabetic} & SDOH &   0.50 &   0.26 &  0.23 &  0.44 &    0.45 &       0.27 &         0.56 \\
        &                               & Tabular &   0.75 &   0.51 &  0.12 &  0.13 &    0.44 &       0.55 &         0.87 \\
        &                               & Tabular+SDOH &   0.75 &   0.51 &  0.10 &  0.10 &    0.30 &       0.52 &         0.90 \\
        &                               & Notes &   0.71 &   0.49 &  0.18 &  0.06 &    0.25 &       0.60 &         0.94 \\
        &                               & Notes+SDOH &   0.70 &   0.47 &  0.21 &  0.16 &    0.40 &       0.47 &         0.84 \\
        &                               & All &   0.76 &   0.56 &  0.18 &  0.07 &    0.30 &       0.61 &         0.93 \\
        &                               & All+SDOH &   0.76 &   0.55 &  0.22 &  0.15 &    0.46 &       0.53 &         0.85 \\
\cline{2-10}
        & \multirow{7}{*}{Elderly Diabetic} & SDOH &   0.49 &   0.35 &  0.16 &  0.51 &    0.48 &       0.33 &         0.49 \\
        &                               & Tabular &   0.73 &   0.56 &  0.11 &  0.26 &    0.61 &       0.55 &         0.74 \\
        &                               & Tabular+SDOH &   0.73 &   0.55 &  0.10 &  0.23 &    0.54 &       0.54 &         0.77 \\
        &                               & Notes &   0.70 &   0.54 &  0.13 &  0.37 &    0.67 &       0.48 &         0.63 \\
        &                               & Notes+SDOH &   0.70 &   0.55 &  0.13 &  0.38 &    0.67 &       0.48 &         0.62 \\
        &                               & All &   0.73 &   0.57 &  0.13 &  0.33 &    0.64 &       0.50 &         0.67 \\
        &                               & All+SDOH &   0.73 &   0.58 &  0.13 &  0.31 &    0.63 &       0.51 &         0.69 \\
\cline{2-10}
        & \multirow{7}{*}{Female Diabetic} & SDOH &   0.50 &   0.24 &  0.21 &  0.21 &    0.21 &       0.25 &         0.79 \\
        &                               & Tabular &   0.77 &   0.48 &  0.14 &  0.21 &    0.57 &       0.47 &         0.79 \\
        &                               & Tabular+SDOH &   0.77 &   0.48 &  0.16 &  0.23 &    0.61 &       0.46 &         0.77 \\
        &                               & Notes &   0.75 &   0.50 &  0.21 &  0.13 &    0.43 &       0.51 &         0.87 \\
        &                               & Notes+SDOH &   0.74 &   0.47 &  0.24 &  0.27 &    0.62 &       0.43 &         0.73 \\
        &                               & All &   0.79 &   0.53 &  0.19 &  0.16 &    0.52 &       0.51 &         0.84 \\
        &                               & All+SDOH &   0.79 &   0.53 &  0.19 &  0.17 &    0.52 &       0.50 &         0.83 \\
\cline{2-10}
        & \multirow{7}{*}{Non-English Speaking Diabetic} & SDOH &   0.54 &   0.27 &  0.24 &  0.40 &    0.39 &       0.25 &         0.60 \\
        &                               & Tabular &   0.74 &   0.47 &  0.14 &  0.24 &    0.55 &       0.44 &         0.76 \\
        &                               & Tabular+SDOH &   0.73 &   0.46 &  0.12 &  0.17 &    0.45 &       0.47 &         0.83 \\
        &                               & Notes &   0.72 &   0.43 &  0.16 &  0.16 &    0.34 &       0.43 &         0.84 \\
        &                               & Notes+SDOH &   0.72 &   0.44 &  0.18 &  0.17 &    0.43 &       0.46 &         0.83 \\
        &                               & All &   0.76 &   0.47 &  0.17 &  0.19 &    0.52 &       0.49 &         0.81 \\
        &                               & All+SDOH &   0.76 &   0.45 &  0.15 &  0.13 &    0.34 &       0.47 &         0.87 \\
\cline{1-10}
\cline{2-10}
\multirow{42}{*}{} & \multirow{7}{*}{All ICU} & SDOH &   0.55 &   0.22 &  0.30 &  0.42 &    0.50 &       0.23 &         0.58 \\
        &                               & Tabular &   0.83 &   0.55 &  0.16 &  0.22 &    0.72 &       0.45 &         0.78 \\
        &                               & Tabular+SDOH &   0.83 &   0.55 &  0.15 &  0.21 &    0.70 &       0.45 &         0.79 \\
        &                               & Notes &   0.82 &   0.53 &  0.17 &  0.18 &    0.64 &       0.46 &         0.82 \\
        &                               & Notes+SDOH &   0.82 &   0.53 &  0.17 &  0.19 &    0.63 &       0.46 &         0.81 \\
        &                               & All &   0.85 &   0.59 &  0.14 &  0.20 &    0.74 &       0.48 &         0.80 \\
        &                               & All+SDOH &   0.85 &   0.60 &  0.14 &  0.20 &    0.73 &       0.48 &         0.80 \\
\cline{2-10}
        & \multirow{7}{*}{All Diabetic} & SDOH &   0.52 &   0.26 &  0.26 &  0.44 &    0.46 &       0.25 &         0.56 \\
        &                               & Tabular &   0.78 &   0.52 &  0.11 &  0.20 &    0.60 &       0.49 &         0.80 \\
        &                               & Tabular+SDOH &   0.78 &   0.52 &  0.10 &  0.19 &    0.57 &       0.49 &         0.81 \\
        &                               & Notes &   0.79 &   0.55 &  0.12 &  0.17 &    0.55 &       0.50 &         0.83 \\
        &                               & Notes+SDOH &   0.79 &   0.55 &  0.11 &  0.17 &    0.55 &       0.51 &         0.83 \\
        &                               & All &   0.81 &   0.57 &  0.09 &  0.17 &    0.62 &       0.53 &         0.83 \\
        &                               & All+SDOH &   0.82 &   0.58 &  0.09 &  0.17 &    0.62 &       0.53 &         0.83 \\
\cline{2-10} \newpage
        & \multirow{7}{*}{Black Diabetic} & SDOH &   0.49 &   0.27 &  0.31 &  0.30 &    0.31 &       0.28 &         0.70 \\
        &                               & Tabular &   0.75 &   0.51 &  0.13 &  0.21 &    0.56 &       0.49 &         0.79 \\
        &                               & Tabular+SDOH &   0.72 &   0.49 &  0.06 &  0.12 &    0.36 &       0.52 &         0.88 \\
XGBoost        &                               & Notes &   0.68 &   0.46 &  0.17 &  0.24 &    0.52 &       0.44 &         0.76 \\
        &                               & Notes+SDOH &   0.70 &   0.52 &  0.07 &  0.10 &    0.36 &       0.55 &         0.90 \\
        &                               & All &   0.76 &   0.55 &  0.05 &  0.10 &    0.39 &       0.59 &         0.90 \\
        &                               & All+SDOH &   0.76 &   0.54 &  0.05 &  0.10 &    0.37 &       0.57 &         0.90 \\
\cline{2-10}
        & \multirow{7}{*}{Elderly Diabetic} & SDOH &   0.51 &   0.35 &  0.27 &  0.43 &    0.48 &       0.36 &         0.57 \\
        &                               & Tabular &   0.73 &   0.56 &  0.07 &  0.25 &    0.57 &       0.55 &         0.75 \\
        &                               & Tabular+SDOH &   0.73 &   0.56 &  0.07 &  0.24 &    0.57 &       0.55 &         0.76 \\
        &                               & Notes &   0.70 &   0.51 &  0.04 &  0.17 &    0.40 &       0.55 &         0.83 \\
        &                               & Notes+SDOH &   0.73 &   0.58 &  0.07 &  0.23 &    0.54 &       0.55 &         0.77 \\
        &                               & All &   0.75 &   0.60 &  0.06 &  0.22 &    0.56 &       0.58 &         0.78 \\
        &                               & All+SDOH &   0.75 &   0.60 &  0.06 &  0.22 &    0.57 &       0.58 &         0.78 \\
\cline{2-10}
        & \multirow{7}{*}{Female Diabetic} & SDOH &   0.49 &   0.24 &  0.25 &  0.40 &    0.39 &       0.24 &         0.60 \\
        &                               & Tabular &   0.77 &   0.49 &  0.19 &  0.33 &    0.72 &       0.41 &         0.67 \\
        &                               & Tabular+SDOH &   0.77 &   0.50 &  0.19 &  0.33 &    0.73 &       0.41 &         0.67 \\
        &                               & Notes &   0.76 &   0.49 &  0.09 &  0.12 &    0.43 &       0.54 &         0.88 \\
        &                               & Notes+SDOH &   0.76 &   0.49 &  0.09 &  0.11 &    0.40 &       0.53 &         0.89 \\
        &                               & All &   0.80 &   0.55 &  0.07 &  0.15 &    0.51 &       0.53 &         0.85 \\
        &                               & All+SDOH &   0.80 &   0.54 &  0.07 &  0.14 &    0.49 &       0.53 &         0.86 \\
\cline{2-10}
        & \multirow{7}{*}{Non-English Speaking Diabetic} & SDOH &   0.50 &   0.25 &  0.22 &  0.26 &    0.22 &       0.22 &         0.74 \\
        &                               & Tabular &   0.75 &   0.48 &  0.14 &  0.27 &    0.62 &       0.44 &         0.73 \\
        &                               & Tabular+SDOH &   0.72 &   0.45 &  0.17 &  0.30 &    0.67 &       0.43 &         0.70 \\
        &                               & Notes &   0.75 &   0.47 &  0.07 &  0.11 &    0.33 &       0.51 &         0.89 \\
        &                               & Notes+SDOH &   0.75 &   0.46 &  0.08 &  0.10 &    0.31 &       0.51 &         0.90 \\
        &                               & All &   0.77 &   0.51 &  0.08 &  0.18 &    0.52 &       0.49 &         0.82 \\
        &                               & All+SDOH &   0.76 &   0.51 &  0.07 &  0.18 &    0.51 &       0.50 &         0.82 \\
\end{longtable}



==> tables/vulnerable_pop_30_day_readm.tex <==
\begin{longtable}{l|llrrrrrrr}
\caption{Comparison of model performance for classifiers trained on different data modalities to predict \textit{30-day readmission} for different patient populations. See \autoref{cohort_stats} for characteristics of the different patient populations.  }
\label{apd:30_day_readm}\\
\toprule
Model        &       Patient                        & Feature Set &  AUROC &  AUPRC &   ECE &   FPR &  Recall &  Precision &  Specificity \\
\midrule
\endfirsthead
\toprule
Model        &       Patient                        & Feature Set &  AUROC &  AUPRC &   ECE &   FPR &  Recall &  Precision &  Specificity \\
\midrule
\endhead
\midrule
\multicolumn{10}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\endlastfoot
\multirow{42}{*}{Logistic Regression} & \multirow{7}{*}{All ICU} & SDOH &   0.53 &   0.07 &  0.44 &  0.53 &    0.59 &       0.07 &         0.47 \\
        &                               & Tabular &   0.66 &   0.11 &  0.40 &  0.37 &    0.61 &       0.10 &         0.63 \\
        &                               & Tabular+SDOH &   0.66 &   0.11 &  0.41 &  0.36 &    0.58 &       0.10 &         0.64 \\
        &                               & Notes &   0.69 &   0.13 &  0.38 &  0.30 &    0.55 &       0.11 &         0.70 \\
        &                               & Notes+SDOH &   0.67 &   0.12 &  0.37 &  0.30 &    0.53 &       0.11 &         0.70 \\
        &                               & All &   0.70 &   0.13 &  0.36 &  0.31 &    0.58 &       0.11 &         0.69 \\
        &                               & All+SDOH &   0.69 &   0.13 &  0.36 &  0.31 &    0.57 &       0.11 &         0.69 \\
\cline{2-10}
        & \multirow{7}{*}{All Diabetic} & SDOH &   0.58 &   0.28 &  0.27 &  0.43 &    0.55 &       0.28 &         0.57 \\
        &                               & Tabular &   0.68 &   0.38 &  0.23 &  0.36 &    0.62 &       0.35 &         0.64 \\
        &                               & Tabular+SDOH &   0.68 &   0.38 &  0.23 &  0.35 &    0.62 &       0.35 &         0.65 \\
        &                               & Notes &   0.71 &   0.42 &  0.19 &  0.28 &    0.58 &       0.39 &         0.72 \\
        &                               & Notes+SDOH &   0.70 &   0.41 &  0.18 &  0.29 &    0.58 &       0.38 &         0.71 \\
        &                               & All &   0.72 &   0.43 &  0.19 &  0.29 &    0.60 &       0.38 &         0.71 \\
        &                               & All+SDOH &   0.72 &   0.43 &  0.18 &  0.29 &    0.60 &       0.39 &         0.71 \\
\cline{2-10}
        & \multirow{7}{*}{Black Diabetic} & SDOH &   0.54 &   0.34 &  0.19 &  0.65 &    0.71 &       0.33 &         0.35 \\
        &                               & Tabular &   0.64 &   0.41 &  0.19 &  0.38 &    0.58 &       0.41 &         0.62 \\
        &                               & Tabular+SDOH &   0.63 &   0.40 &  0.19 &  0.48 &    0.68 &       0.39 &         0.52 \\
        &                               & Notes &   0.63 &   0.44 &  0.14 &  0.33 &    0.52 &       0.42 &         0.67 \\
        &                               & Notes+SDOH &   0.61 &   0.42 &  0.13 &  0.25 &    0.39 &       0.42 &         0.75 \\
        &                               & All &   0.64 &   0.41 &  0.19 &  0.38 &    0.58 &       0.41 &         0.62 \\
        &                               & All+SDOH &   0.63 &   0.40 &  0.19 &  0.47 &    0.68 &       0.39 &         0.53 \\
\cline{2-10}
        & \multirow{7}{*}{Elderly Diabetic} & SDOH &   0.60 &   0.30 &  0.27 &  0.41 &    0.59 &       0.29 &         0.59 \\
        &                               & Tabular &   0.65 &   0.35 &  0.24 &  0.36 &    0.57 &       0.32 &         0.64 \\
        &                               & Tabular+SDOH &   0.64 &   0.35 &  0.25 &  0.34 &    0.58 &       0.33 &         0.66 \\
        &                               & Notes &   0.66 &   0.35 &  0.19 &  0.25 &    0.47 &       0.35 &         0.75 \\
        &                               & Notes+SDOH &   0.65 &   0.35 &  0.18 &  0.27 &    0.48 &       0.34 &         0.73 \\
        &                               & All &   0.67 &   0.37 &  0.18 &  0.26 &    0.51 &       0.36 &         0.74 \\
        &                               & All+SDOH &   0.64 &   0.35 &  0.25 &  0.34 &    0.58 &       0.34 &         0.66 \\
\cline{2-10}
        & \multirow{7}{*}{Female Diabetic} & SDOH &   0.58 &   0.32 &  0.25 &  0.40 &    0.55 &       0.31 &         0.60 \\
        &                               & Tabular &   0.68 &   0.40 &  0.22 &  0.35 &    0.60 &       0.36 &         0.65 \\
        &                               & Tabular+SDOH &   0.65 &   0.39 &  0.23 &  0.34 &    0.54 &       0.34 &         0.66 \\
        &                               & Notes &   0.69 &   0.42 &  0.18 &  0.28 &    0.54 &       0.39 &         0.72 \\
        &                               & Notes+SDOH &   0.68 &   0.41 &  0.17 &  0.28 &    0.55 &       0.39 &         0.72 \\
        &                               & All &   0.70 &   0.42 &  0.17 &  0.29 &    0.57 &       0.40 &         0.71 \\
        &                               & All+SDOH &   0.69 &   0.41 &  0.17 &  0.28 &    0.56 &       0.40 &         0.72 \\
\cline{2-10}
        & \multirow{7}{*}{Non-English Speaking Diabetic} & SDOH &   0.64 &   0.37 &  0.27 &  0.57 &    0.76 &       0.30 &         0.43 \\
        &                               & Tabular &   0.68 &   0.41 &  0.24 &  0.39 &    0.66 &       0.35 &         0.61 \\
        &                               & Tabular+SDOH &   0.69 &   0.45 &  0.25 &  0.36 &    0.60 &       0.35 &         0.64 \\
        &                               & Notes &   0.72 &   0.44 &  0.18 &  0.23 &    0.54 &       0.43 &         0.77 \\
        &                               & Notes+SDOH &   0.66 &   0.38 &  0.12 &  0.20 &    0.38 &       0.38 &         0.80 \\
        &                               & All &   0.68 &   0.41 &  0.24 &  0.39 &    0.66 &       0.35 &         0.61 \\
        &                               & All+SDOH &   0.69 &   0.45 &  0.25 &  0.36 &    0.60 &       0.35 &         0.64 \\
\cline{1-10}
\cline{2-10}
\multirow{42}{*}{} & \multirow{7}{*}{All ICU} & SDOH &   0.53 &   0.07 &  0.43 &  0.41 &    0.46 &       0.07 &         0.59 \\
        &                               & Tabular &   0.66 &   0.11 &  0.40 &  0.33 &    0.56 &       0.10 &         0.67 \\
        &                               & Tabular+SDOH &   0.66 &   0.11 &  0.36 &  0.18 &    0.35 &       0.11 &         0.82 \\
        &                               & Notes &   0.66 &   0.12 &  0.38 &  0.17 &    0.34 &       0.12 &         0.83 \\
        &                               & Notes+SDOH &   0.66 &   0.12 &  0.41 &  0.27 &    0.49 &       0.11 &         0.73 \\
        &                               & All &   0.68 &   0.13 &  0.41 &  0.28 &    0.54 &       0.11 &         0.72 \\
        &                               & All+SDOH &   0.68 &   0.13 &  0.41 &  0.28 &    0.54 &       0.11 &         0.72 \\
\cline{2-10}
        & \multirow{7}{*}{All Diabetic} & SDOH &   0.58 &   0.29 &  0.27 &  0.36 &    0.47 &       0.28 &         0.64 \\
        &                               & Tabular &   0.67 &   0.37 &  0.20 &  0.28 &    0.49 &       0.35 &         0.72 \\
        &                               & Tabular+SDOH &   0.68 &   0.38 &  0.20 &  0.26 &    0.49 &       0.36 &         0.74 \\
Random Forest        &                               & Notes &   0.69 &   0.41 &  0.22 &  0.32 &    0.59 &       0.35 &         0.68 \\
        &                               & Notes+SDOH &   0.69 &   0.41 &  0.22 &  0.31 &    0.58 &       0.36 &         0.69 \\
        &                               & All &   0.69 &   0.41 &  0.21 &  0.27 &    0.53 &       0.38 &         0.73 \\
        &                               & All+SDOH &   0.70 &   0.41 &  0.22 &  0.29 &    0.56 &       0.37 &         0.71 \\
\cline{2-10}
        & \multirow{7}{*}{Black Diabetic} & SDOH &   0.56 &   0.34 &  0.18 &  0.48 &    0.55 &       0.34 &         0.52 \\
        &                               & Tabular &   0.64 &   0.42 &  0.10 &  0.19 &    0.32 &       0.43 &         0.81 \\
        &                               & Tabular+SDOH &   0.64 &   0.43 &  0.10 &  0.15 &    0.28 &       0.46 &         0.85 \\
        &                               & Notes &   0.64 &   0.46 &  0.15 &  0.22 &    0.40 &       0.45 &         0.78 \\
        &                               & Notes+SDOH &   0.64 &   0.46 &  0.14 &  0.16 &    0.31 &       0.47 &         0.84 \\
        &                               & All &   0.65 &   0.47 &  0.18 &  0.31 &    0.49 &       0.42 &         0.69 \\
        &                               & All+SDOH &   0.66 &   0.47 &  0.14 &  0.15 &    0.31 &       0.49 &         0.85 \\
\cline{2-10}
        & \multirow{7}{*}{Elderly Diabetic} & SDOH &   0.60 &   0.30 &  0.27 &  0.40 &    0.56 &       0.29 &         0.60 \\
        &                               & Tabular &   0.63 &   0.35 &  0.22 &  0.29 &    0.49 &       0.33 &         0.71 \\
        &                               & Tabular+SDOH &   0.65 &   0.35 &  0.23 &  0.27 &    0.48 &       0.34 &         0.73 \\
        &                               & Notes &   0.64 &   0.35 &  0.20 &  0.15 &    0.32 &       0.38 &         0.85 \\
        &                               & Notes+SDOH &   0.65 &   0.35 &  0.20 &  0.15 &    0.34 &       0.39 &         0.85 \\
        &                               & All &   0.66 &   0.36 &  0.19 &  0.12 &    0.32 &       0.44 &         0.88 \\
        &                               & All+SDOH &   0.67 &   0.37 &  0.21 &  0.16 &    0.37 &       0.40 &         0.84 \\
\cline{2-10}
        & \multirow{7}{*}{Female Diabetic} & SDOH &   0.59 &   0.32 &  0.25 &  0.38 &    0.53 &       0.32 &         0.62 \\
        &                               & Tabular &   0.65 &   0.38 &  0.21 &  0.30 &    0.47 &       0.35 &         0.70 \\
        &                               & Tabular+SDOH &   0.65 &   0.39 &  0.21 &  0.29 &    0.46 &       0.35 &         0.71 \\
        &                               & Notes &   0.69 &   0.44 &  0.23 &  0.30 &    0.56 &       0.38 &         0.70 \\
        &                               & Notes+SDOH &   0.69 &   0.45 &  0.23 &  0.29 &    0.55 &       0.39 &         0.71 \\
        &                               & All &   0.69 &   0.44 &  0.19 &  0.16 &    0.40 &       0.45 &         0.84 \\
        &                               & All+SDOH &   0.70 &   0.45 &  0.25 &  0.31 &    0.58 &       0.38 &         0.69 \\
\cline{2-10}
        & \multirow{7}{*}{Non-English Speaking Diabetic} & SDOH &   0.63 &   0.37 &  0.25 &  0.41 &    0.58 &       0.31 &         0.59 \\
        &                               & Tabular &   0.68 &   0.42 &  0.18 &  0.26 &    0.50 &       0.38 &         0.74 \\
        &                               & Tabular+SDOH &   0.69 &   0.44 &  0.24 &  0.34 &    0.64 &       0.38 &         0.66 \\
        &                               & Notes &   0.72 &   0.45 &  0.17 &  0.09 &    0.29 &       0.51 &         0.91 \\
        &                               & Notes+SDOH &   0.72 &   0.48 &  0.17 &  0.06 &    0.26 &       0.58 &         0.94 \\
        &                               & All &   0.73 &   0.48 &  0.21 &  0.22 &    0.55 &       0.44 &         0.78 \\
        &                               & All+SDOH &   0.73 &   0.48 &  0.21 &  0.20 &    0.54 &       0.46 &         0.80 \\
\cline{1-10}
\cline{2-10}
\multirow{42}{*}{} & \multirow{7}{*}{All ICU} & SDOH &   0.53 &   0.07 &  0.43 &  0.44 &    0.49 &       0.07 &         0.56 \\
        &                               & Tabular &   0.67 &   0.11 &  0.38 &  0.34 &    0.56 &       0.10 &         0.66 \\
        &                               & Tabular+SDOH &   0.67 &   0.11 &  0.37 &  0.33 &    0.56 &       0.10 &         0.67 \\
        &                               & Notes &   0.68 &   0.13 &  0.36 &  0.24 &    0.46 &       0.11 &         0.76 \\
        &                               & Notes+SDOH &   0.68 &   0.13 &  0.36 &  0.24 &    0.47 &       0.11 &         0.76 \\
        &                               & All &   0.70 &   0.13 &  0.35 &  0.27 &    0.54 &       0.12 &         0.73 \\
        &                               & All+SDOH &   0.70 &   0.13 &  0.35 &  0.27 &    0.54 &       0.12 &         0.73 \\
\cline{2-10}
        & \multirow{7}{*}{All Diabetic} & SDOH &   0.58 &   0.28 &  0.26 &  0.41 &    0.54 &       0.28 &         0.59 \\
        &                               & Tabular &   0.68 &   0.37 &  0.22 &  0.36 &    0.60 &       0.34 &         0.64 \\
        &                               & Tabular+SDOH &   0.68 &   0.38 &  0.21 &  0.35 &    0.61 &       0.34 &         0.65 \\
XGBoost        &                               & Notes &   0.71 &   0.43 &  0.21 &  0.30 &    0.61 &       0.38 &         0.70 \\
        &                               & Notes+SDOH &   0.71 &   0.43 &  0.21 &  0.30 &    0.61 &       0.38 &         0.70 \\
        &                               & All &   0.72 &   0.43 &  0.20 &  0.31 &    0.61 &       0.37 &         0.69 \\
        &                               & All+SDOH &   0.72 &   0.43 &  0.20 &  0.31 &    0.61 &       0.38 &         0.69 \\
\cline{2-10} \newpage
        & \multirow{7}{*}{Black Diabetic} & SDOH &   0.52 &   0.34 &  0.27 &  0.33 &    0.41 &       0.36 &         0.67 \\
        &                               & Tabular &   0.65 &   0.44 &  0.15 &  0.35 &    0.56 &       0.42 &         0.65 \\
        &                               & Tabular+SDOH &   0.66 &   0.44 &  0.14 &  0.31 &    0.55 &       0.44 &         0.69 \\
        &                               & Notes &   0.64 &   0.45 &  0.13 &  0.26 &    0.44 &       0.43 &         0.74 \\
        &                               & Notes+SDOH &   0.65 &   0.46 &  0.12 &  0.25 &    0.47 &       0.45 &         0.75 \\
        &                               & All &   0.66 &   0.47 &  0.13 &  0.25 &    0.47 &       0.45 &         0.75 \\
        &                               & All+SDOH &   0.66 &   0.47 &  0.13 &  0.25 &    0.46 &       0.45 &         0.75 \\
\cline{2-10}
        & \multirow{7}{*}{Elderly Diabetic} & SDOH &   0.58 &   0.28 &  0.26 &  0.42 &    0.55 &       0.27 &         0.58 \\
        &                               & Tabular &   0.64 &   0.34 &  0.23 &  0.36 &    0.57 &       0.32 &         0.64 \\
        &                               & Tabular+SDOH &   0.65 &   0.35 &  0.23 &  0.36 &    0.57 &       0.32 &         0.64 \\
        &                               & Notes &   0.66 &   0.34 &  0.17 &  0.21 &    0.41 &       0.36 &         0.79 \\
        &                               & Notes+SDOH &   0.67 &   0.36 &  0.08 &  0.11 &    0.28 &       0.43 &         0.89 \\
        &                               & All &   0.67 &   0.37 &  0.22 &  0.31 &    0.58 &       0.36 &         0.69 \\
        &                               & All+SDOH &   0.68 &   0.37 &  0.08 &  0.11 &    0.29 &       0.44 &         0.89 \\
\cline{2-10}
        & \multirow{7}{*}{Female Diabetic} & SDOH &   0.59 &   0.32 &  0.24 &  0.34 &    0.50 &       0.33 &         0.66 \\
        &                               & Tabular &   0.67 &   0.39 &  0.22 &  0.37 &    0.57 &       0.34 &         0.63 \\
        &                               & Tabular+SDOH &   0.67 &   0.40 &  0.22 &  0.36 &    0.59 &       0.35 &         0.64 \\
        &                               & Notes &   0.70 &   0.44 &  0.18 &  0.26 &    0.55 &       0.41 &         0.74 \\
        &                               & Notes+SDOH &   0.69 &   0.42 &  0.10 &  0.15 &    0.40 &       0.46 &         0.85 \\
        &                               & All &   0.71 &   0.44 &  0.09 &  0.15 &    0.39 &       0.46 &         0.85 \\
        &                               & All+SDOH &   0.71 &   0.43 &  0.09 &  0.16 &    0.39 &       0.45 &         0.84 \\
\cline{2-10}
        & \multirow{7}{*}{Non-English Speaking Diabetic} & SDOH &   0.57 &   0.30 &  0.20 &  0.27 &    0.38 &       0.31 &         0.73 \\
        &                               & Tabular &   0.69 &   0.43 &  0.21 &  0.36 &    0.61 &       0.35 &         0.64 \\
        &                               & Tabular+SDOH &   0.69 &   0.45 &  0.23 &  0.36 &    0.61 &       0.35 &         0.64 \\
        &                               & Notes &   0.70 &   0.45 &  0.14 &  0.19 &    0.48 &       0.45 &         0.81 \\
        &                               & Notes+SDOH &   0.70 &   0.45 &  0.14 &  0.18 &    0.47 &       0.46 &         0.82 \\
        &                               & All &   0.70 &   0.45 &  0.16 &  0.23 &    0.50 &       0.41 &         0.77 \\
        &                               & All+SDOH &   0.70 &   0.46 &  0.16 &  0.23 &    0.50 &       0.41 &         0.77 \\
\end{longtable}



==> tables/vulnerable_pop_in_hosp_mort.tex <==
\begin{longtable}{l|llrrrrrrr}
\caption{Comparison of model performance for classifiers trained on different data modalities to predict \textit{in-hospital mortality} for different patient populations. See \autoref{cohort_stats} for characteristics of the different patient populations. }
\label{apd:expire_flag}\\
\toprule
Model        &       Patient                        & Feature Set &  AUROC &  AUPRC &   ECE &   FPR &  Recall &  Precision &  Specificity \\
\midrule
\endfirsthead
\toprule
Model        &       Patient                        & Feature Set &  AUROC &  AUPRC &   ECE &   FPR &  Recall &  Precision &  Specificity \\
\midrule
\endhead
\midrule
\multicolumn{10}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\endlastfoot
\multirow{42}{*}{Logistic Regression} & \multirow{7}{*}{All ICU} & SDOH &   0.51 &   0.09 &  0.41 &  0.40 &    0.41 &       0.09 &         0.60 \\
        &                               & Tabular &   0.85 &   0.39 &  0.26 &  0.22 &    0.76 &       0.25 &         0.78 \\
        &                               & Tabular+SDOH &   0.85 &   0.39 &  0.26 &  0.22 &    0.77 &       0.25 &         0.78 \\
        &                               & Notes &   0.86 &   0.38 &  0.21 &  0.18 &    0.69 &       0.27 &         0.82 \\
        &                               & Notes+SDOH &   0.85 &   0.37 &  0.22 &  0.20 &    0.71 &       0.25 &         0.80 \\
        &                               & All &   0.90 &   0.49 &  0.18 &  0.16 &    0.80 &       0.31 &         0.84 \\
        &                               & All+SDOH &   0.90 &   0.48 &  0.19 &  0.17 &    0.81 &       0.30 &         0.83 \\
\cline{2-10}
        & \multirow{7}{*}{All Diabetic} & SDOH &   0.52 &   0.09 &  0.40 &  0.39 &    0.41 &       0.09 &         0.61 \\
        &                               & Tabular &   0.84 &   0.37 &  0.26 &  0.22 &    0.73 &       0.25 &         0.78 \\
        &                               & Tabular+SDOH &   0.84 &   0.36 &  0.26 &  0.22 &    0.72 &       0.25 &         0.78 \\
        &                               & Notes &   0.82 &   0.32 &  0.21 &  0.16 &    0.62 &       0.27 &         0.84 \\
        &                               & Notes+SDOH &   0.82 &   0.32 &  0.14 &  0.13 &    0.54 &       0.28 &         0.87 \\
        &                               & All &   0.88 &   0.43 &  0.16 &  0.14 &    0.69 &       0.32 &         0.86 \\
        &                               & All+SDOH &   0.87 &   0.42 &  0.16 &  0.14 &    0.70 &       0.32 &         0.86 \\
\cline{2-10}
        & \multirow{7}{*}{Black Diabetic} & SDOH &   0.51 &   0.08 &  0.41 &  0.44 &    0.42 &       0.07 &         0.56 \\
        &                               & Tabular &   0.85 &   0.42 &  0.25 &  0.19 &    0.71 &       0.23 &         0.81 \\
        &                               & Tabular+SDOH &   0.86 &   0.42 &  0.31 &  0.17 &    0.75 &       0.26 &         0.83 \\
        &                               & Notes &   0.78 &   0.19 &  0.11 &  0.05 &    0.16 &       0.18 &         0.95 \\
        &                               & Notes+SDOH &   0.71 &   0.14 &  0.10 &  0.06 &    0.17 &       0.19 &         0.94 \\
        &                               & All &   0.85 &   0.41 &  0.25 &  0.19 &    0.72 &       0.22 &         0.81 \\
        &                               & All+SDOH &   0.86 &   0.42 &  0.31 &  0.17 &    0.73 &       0.25 &         0.83 \\
\cline{2-10}
        & \multirow{7}{*}{Elderly Diabetic} & SDOH &   0.51 &   0.14 &  0.37 &  0.47 &    0.50 &       0.14 &         0.53 \\
        &                               & Tabular &   0.79 &   0.39 &  0.27 &  0.28 &    0.71 &       0.28 &         0.72 \\
        &                               & Tabular+SDOH &   0.79 &   0.39 &  0.27 &  0.26 &    0.71 &       0.28 &         0.74 \\
        &                               & Notes &   0.76 &   0.31 &  0.23 &  0.18 &    0.54 &       0.30 &         0.82 \\
        &                               & Notes+SDOH &   0.75 &   0.31 &  0.12 &  0.11 &    0.37 &       0.32 &         0.89 \\
        &                               & All &   0.82 &   0.42 &  0.11 &  0.13 &    0.56 &       0.38 &         0.87 \\
        &                               & All+SDOH &   0.82 &   0.43 &  0.11 &  0.13 &    0.54 &       0.37 &         0.87 \\
\cline{2-10}
        & \multirow{7}{*}{Female Diabetic} & SDOH &   0.50 &   0.09 &  0.41 &  1.00 &    1.00 &       0.09 &         0.00 \\
        &                               & Tabular &   0.85 &   0.38 &  0.26 &  0.21 &    0.72 &       0.26 &         0.79 \\
        &                               & Tabular+SDOH &   0.85 &   0.37 &  0.25 &  0.21 &    0.72 &       0.26 &         0.79 \\
        &                               & Notes &   0.82 &   0.36 &  0.22 &  0.12 &    0.57 &       0.32 &         0.88 \\
        &                               & Notes+SDOH &   0.78 &   0.30 &  0.11 &  0.08 &    0.40 &       0.33 &         0.92 \\
        &                               & All &   0.88 &   0.43 &  0.16 &  0.13 &    0.70 &       0.35 &         0.87 \\
        &                               & All+SDOH &   0.86 &   0.39 &  0.09 &  0.09 &    0.53 &       0.36 &         0.91 \\
\cline{2-10}
        & \multirow{7}{*}{Non-English Speaking Diabetic} & SDOH &   0.57 &   0.15 &  0.40 &  0.39 &    0.53 &       0.13 &         0.61 \\
        &                               & Tabular &   0.83 &   0.41 &  0.26 &  0.24 &    0.80 &       0.26 &         0.76 \\
        &                               & Tabular+SDOH &   0.81 &   0.37 &  0.33 &  0.22 &    0.67 &       0.24 &         0.78 \\
        &                               & Notes &   0.80 &   0.31 &  0.12 &  0.06 &    0.28 &       0.35 &         0.94 \\
        &                               & Notes+SDOH &   0.76 &   0.31 &  0.11 &  0.08 &    0.34 &       0.32 &         0.92 \\
        &                               & All &   0.84 &   0.43 &  0.24 &  0.22 &    0.78 &       0.28 &         0.78 \\
        &                               & All+SDOH &   0.80 &   0.36 &  0.32 &  0.22 &    0.67 &       0.24 &         0.78 \\
\cline{1-10}
\cline{2-10}
\multirow{42}{*}{Random Forest} & \multirow{7}{*}{All ICU} & SDOH &   0.52 &   0.09 &  0.41 &  0.45 &    0.48 &       0.09 &         0.55 \\
        &                               & Tabular &   0.84 &   0.38 &  0.23 &  0.15 &    0.63 &       0.28 &         0.85 \\
        &                               & Tabular+SDOH &   0.84 &   0.38 &  0.24 &  0.15 &    0.62 &       0.28 &         0.85 \\
        &                               & Notes &   0.77 &   0.25 &  0.34 &  0.25 &    0.65 &       0.19 &         0.75 \\
        &                               & Notes+SDOH &   0.77 &   0.26 &  0.34 &  0.24 &    0.64 &       0.19 &         0.76 \\
        &                               & All &   0.86 &   0.36 &  0.30 &  0.17 &    0.68 &       0.27 &         0.83 \\
        &                               & All+SDOH &   0.85 &   0.36 &  0.31 &  0.17 &    0.69 &       0.27 &         0.83 \\
\cline{2-10}
        & \multirow{7}{*}{All Diabetic} & SDOH &   0.51 &   0.09 &  0.41 &  0.42 &    0.40 &       0.09 &         0.58 \\
        &                               & Tabular &   0.83 &   0.36 &  0.18 &  0.09 &    0.48 &       0.34 &         0.91 \\
        &                               & Tabular+SDOH &   0.83 &   0.35 &  0.19 &  0.09 &    0.47 &       0.35 &         0.91 \\
        &                               & Notes &   0.75 &   0.24 &  0.33 &  0.20 &    0.52 &       0.20 &         0.80 \\
        &                               & Notes+SDOH &   0.75 &   0.24 &  0.33 &  0.20 &    0.55 &       0.21 &         0.80 \\
        &                               & All &   0.84 &   0.36 &  0.27 &  0.11 &    0.52 &       0.32 &         0.89 \\
        &                               & All+SDOH &   0.84 &   0.35 &  0.29 &  0.13 &    0.60 &       0.30 &         0.87 \\
\cline{2-10}
        & \multirow{7}{*}{Black Diabetic} & SDOH &   0.48 &   0.07 &  0.29 &  0.27 &    0.19 &       0.05 &         0.73 \\
        &                               & Tabular &   0.86 &   0.45 &  0.14 &  0.05 &    0.49 &       0.45 &         0.95 \\
        &                               & Tabular+SDOH &   0.86 &   0.43 &  0.11 &  0.01 &    0.21 &       0.64 &         0.99 \\
Random Forest        &                               & Notes &   0.72 &   0.15 &  0.22 &  0.00 &    0.00 &       0.00 &         1.00 \\
        &                               & Notes+SDOH &   0.72 &   0.16 &  0.21 &  0.00 &    0.00 &       0.00 &         1.00 \\
        &                               & All &   0.86 &   0.37 &  0.18 &  0.00 &    0.02 &       0.50 &         1.00 \\
        &                               & All+SDOH &   0.85 &   0.35 &  0.18 &  0.00 &    0.02 &       0.50 &         1.00 \\
\cline{2-10}
        & \multirow{7}{*}{Elderly Diabetic} & SDOH &   0.51 &   0.13 &  0.37 &  0.40 &    0.43 &       0.14 &         0.60 \\
        &                               & Tabular &   0.76 &   0.36 &  0.16 &  0.08 &    0.32 &       0.38 &         0.92 \\
        &                               & Tabular+SDOH &   0.76 &   0.37 &  0.16 &  0.07 &    0.28 &       0.38 &         0.93 \\
        &                               & Notes &   0.70 &   0.26 &  0.28 &  0.13 &    0.30 &       0.25 &         0.87 \\
        &                               & Notes+SDOH &   0.70 &   0.26 &  0.26 &  0.09 &    0.21 &       0.25 &         0.91 \\
        &                               & All &   0.79 &   0.37 &  0.26 &  0.08 &    0.35 &       0.37 &         0.92 \\
        &                               & All+SDOH &   0.78 &   0.37 &  0.24 &  0.06 &    0.29 &       0.41 &         0.94 \\
\cline{2-10}
        & \multirow{7}{*}{Female Diabetic} & SDOH &   0.50 &   0.09 &  0.28 &  0.26 &    0.25 &       0.09 &         0.74 \\
        &                               & Tabular &   0.84 &   0.37 &  0.13 &  0.06 &    0.35 &       0.38 &         0.94 \\
        &                               & Tabular+SDOH &   0.83 &   0.37 &  0.15 &  0.05 &    0.33 &       0.40 &         0.95 \\
        &                               & Notes &   0.73 &   0.25 &  0.31 &  0.05 &    0.21 &       0.28 &         0.95 \\
        &                               & Notes+SDOH &   0.73 &   0.25 &  0.31 &  0.05 &    0.22 &       0.31 &         0.95 \\
        &                               & All &   0.84 &   0.37 &  0.27 &  0.05 &    0.33 &       0.40 &         0.95 \\
        &                               & All+SDOH &   0.85 &   0.40 &  0.27 &  0.05 &    0.36 &       0.41 &         0.95 \\
\cline{2-10}
        & \multirow{7}{*}{Non-English Speaking Diabetic} & SDOH &   0.57 &   0.15 &  0.39 &  0.34 &    0.50 &       0.14 &         0.66 \\
        &                               & Tabular &   0.80 &   0.37 &  0.16 &  0.08 &    0.36 &       0.34 &         0.92 \\
        &                               & Tabular+SDOH &   0.80 &   0.34 &  0.12 &  0.03 &    0.25 &       0.45 &         0.97 \\
        &                               & Notes &   0.74 &   0.23 &  0.30 &  0.06 &    0.16 &       0.22 &         0.94 \\
        &                               & Notes+SDOH &   0.75 &   0.23 &  0.22 &  0.00 &    0.01 &       1.00 &         1.00 \\
        &                               & All &   0.82 &   0.38 &  0.22 &  0.02 &    0.12 &       0.47 &         0.98 \\
        &                               & All+SDOH &   0.82 &   0.36 &  0.18 &  0.01 &    0.03 &       0.40 &         0.99 \\
\cline{1-10}
\cline{2-10}
\multirow{42}{*}{} & \multirow{7}{*}{All ICU} & SDOH &   0.52 &   0.09 &  0.41 &  0.38 &    0.40 &       0.09 &         0.62 \\
        &                               & Tabular &   0.86 &   0.42 &  0.14 &  0.11 &    0.60 &       0.35 &         0.89 \\
        &                               & Tabular+SDOH &   0.86 &   0.42 &  0.13 &  0.10 &    0.57 &       0.35 &         0.90 \\
        &                               & Notes &   0.84 &   0.38 &  0.18 &  0.10 &    0.54 &       0.33 &         0.90 \\
        &                               & Notes+SDOH &   0.84 &   0.38 &  0.18 &  0.10 &    0.53 &       0.33 &         0.90 \\
        &                               & All &   0.90 &   0.49 &  0.11 &  0.09 &    0.63 &       0.40 &         0.91 \\
        &                               & All+SDOH &   0.90 &   0.49 &  0.11 &  0.09 &    0.63 &       0.40 &         0.91 \\
\cline{2-10}
        & \multirow{7}{*}{All Diabetic} & SDOH &   0.49 &   0.09 &  0.28 &  0.22 &    0.20 &       0.08 &         0.78 \\
        &                               & Tabular &   0.84 &   0.38 &  0.10 &  0.07 &    0.46 &       0.39 &         0.93 \\
        &                               & Tabular+SDOH &   0.84 &   0.38 &  0.09 &  0.07 &    0.45 &       0.39 &         0.93 \\
        &                               & Notes &   0.81 &   0.30 &  0.12 &  0.05 &    0.30 &       0.37 &         0.95 \\
        &                               & Notes+SDOH &   0.81 &   0.30 &  0.12 &  0.05 &    0.30 &       0.36 &         0.95 \\
        &                               & All &   0.88 &   0.44 &  0.07 &  0.05 &    0.47 &       0.45 &         0.95 \\
        &                               & All+SDOH &   0.88 &   0.45 &  0.07 &  0.05 &    0.46 &       0.45 &         0.95 \\
\cline{2-10} \newpage
        & \multirow{7}{*}{Black Diabetic} & SDOH &   0.44 &   0.07 &  0.28 &  0.34 &    0.29 &       0.06 &         0.66 \\
      &                               & Tabular &   0.85 &   0.46 &  0.06 &  0.04 &    0.48 &       0.47 &         0.96 \\
        &                               & Tabular+SDOH &   0.84 &   0.45 &  0.05 &  0.03 &    0.38 &       0.46 &         0.97 \\
        &                               & Notes &   0.73 &   0.17 &  0.15 &  0.06 &    0.21 &       0.21 &         0.94 \\
 XGBoost         &                               & Notes+SDOH &   0.73 &   0.16 &  0.17 &  0.04 &    0.10 &       0.15 &         0.96 \\
        &                               & All &   0.87 &   0.45 &  0.03 &  0.01 &    0.32 &       0.64 &         0.99 \\
        &                               & All+SDOH &   0.88 &   0.45 &  0.04 &  0.01 &    0.28 &       0.64 &         0.99 \\
\cline{2-10}
        & \multirow{7}{*}{Elderly Diabetic} & SDOH &   0.53 &   0.14 &  0.25 &  0.21 &    0.18 &       0.11 &         0.79 \\
        &                               & Tabular &   0.78 &   0.37 &  0.09 &  0.09 &    0.39 &       0.39 &         0.91 \\
        &                               & Tabular+SDOH &   0.78 &   0.38 &  0.08 &  0.08 &    0.38 &       0.40 &         0.92 \\
        &                               & Notes &   0.73 &   0.30 &  0.07 &  0.04 &    0.20 &       0.40 &         0.96 \\
        &                               & Notes+SDOH &   0.73 &   0.31 &  0.07 &  0.05 &    0.19 &       0.36 &         0.95 \\
        &                               & All &   0.81 &   0.41 &  0.05 &  0.06 &    0.32 &       0.42 &         0.94 \\
        &                               & All+SDOH &   0.81 &   0.40 &  0.05 &  0.06 &    0.33 &       0.44 &         0.94 \\
\cline{2-10}
        & \multirow{7}{*}{Female Diabetic} & SDOH &   0.49 &   0.10 &  0.24 &  0.15 &    0.14 &       0.09 &         0.85 \\
        &                               & Tabular &   0.84 &   0.39 &  0.06 &  0.06 &    0.38 &       0.41 &         0.94 \\
        &                               & Tabular+SDOH &   0.84 &   0.39 &  0.06 &  0.05 &    0.37 &       0.41 &         0.95 \\
        &                               & Notes &   0.77 &   0.29 &  0.07 &  0.02 &    0.12 &       0.44 &         0.98 \\
        &                               & Notes+SDOH &   0.78 &   0.29 &  0.07 &  0.01 &    0.14 &       0.48 &         0.99 \\
        &                               & All &   0.88 &   0.42 &  0.04 &  0.03 &    0.34 &       0.50 &         0.97 \\
        &                               & All+SDOH &   0.88 &   0.43 &  0.04 &  0.03 &    0.34 &       0.52 &         0.97 \\
\cline{2-10}
        & \multirow{7}{*}{Non-English Speaking Diabetic} & SDOH &   0.55 &   0.14 &  0.30 &  0.16 &    0.25 &       0.14 &         0.84 \\
        &                               & Tabular &   0.81 &   0.32 &  0.20 &  0.16 &    0.61 &       0.29 &         0.84 \\
        &                               & Tabular+SDOH &   0.81 &   0.31 &  0.19 &  0.16 &    0.58 &       0.28 &         0.84 \\
        &                               & Notes &   0.75 &   0.22 &  0.15 &  0.08 &    0.25 &       0.25 &         0.92 \\
        &                               & Notes+SDOH &   0.75 &   0.22 &  0.16 &  0.09 &    0.22 &       0.22 &         0.91 \\
        &                               & All &   0.82 &   0.32 &  0.16 &  0.10 &    0.45 &       0.33 &         0.90 \\
        &                               & All+SDOH &   0.83 &   0.33 &  0.12 &  0.09 &    0.40 &       0.33 &         0.91 \\
\end{longtable}



==> tables/vulnerable_pop_main.tex <==
\begin{table}[!b]
\caption{Comparison of the performance of XGBoost models trained on \texttt{Notes} and \texttt{Notes+SDOH} to predict one-year mortality for different diabetic patient populations. The effect of incorporating SDOH is larger on the more vulnerable populations (i.e. Black diabetic patients and elderly diabetic patients). See \autoref{cohort_stats} for characteristics of the different patient populations. Values in bold indicate significantly better performance, evaluated using a 1000-sample bootstrap hypothesis test at the 5\% significance level.}
\label{tab:all_vs_black_diabetic}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}llP{10mm}P{10mm}P{10mm}P{14mm}@{}}
\toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}} Patient \\ Population\end{tabular}}             & \multirow{2}{*}{Feature Set}  & ECE & FPR & Recall & Specificity \\ 
& & ($\downarrow$) & ($\downarrow$) & ($\uparrow$) & ($\uparrow$) \\\midrule
\multirow{2}{*}{All Diabetic}                  & \texttt{Notes}                        & 0.12          & 0.17 & 0.55           & 0.83          \\
                                               & \texttt{Notes+SDOH}                   & 0.11          & 0.17 & 0.55           & 0.83          \\ \midrule
\multirow{2}{*}{Black Diabetic}                & \texttt{Notes}                        & 0.17          & 0.24 & \textbf{0.52}    & 0.76          \\
                                               & \texttt{Notes+SDOH}                   & \textbf{0.08} & \textbf{0.11} & 0.36    & \textbf{0.89} \\ \midrule
\multirow{2}{*}{Elderly Diabetic}              & \texttt{Notes}                        & \textbf{0.04} & \textbf{0.17} & 0.40     & \textbf{0.83} \\
                                               & \texttt{Notes+SDOH}                   & 0.07          & 0.23 & \textbf{0.54} & 0.55    \\  \bottomrule
\end{tabular}%
}
\end{table}

